Actris 2.0: Asynchronous Session-Type Based Reasoning in Separation Logic

Message passing is a useful abstraction for implementing concurrent programs. For real-world systems, however, it is often combined with other programming and concurrency paradigms, such as higher-order functions, mutable state, shared-memory concurrency, and locks. We present Actris: a logic for proving functional correctness of programs that use a combination of the aforementioned features. Actris combines the power of modern concurrent separation logics with a first-class protocol mechanism -- based on session types -- for reasoning about message passing in the presence of other concurrency paradigms. We show that Actris provides a suitable level of abstraction by proving functional correctness of a variety of examples, including a channel-based merge sort, a channel-based load-balancing mapper, and a variant of the map-reduce model, using concise specifications. While Actris was already presented in a conference paper (POPL'20), this paper expands the prior presentation significantly. Moreover, it extends Actris to Actris 2.0 with a notion of subprotocols -- based on session-type subtyping -- that permits additional flexibility when composing channel endpoints, and that takes full advantage of the asynchronous semantics of message passing in Actris. Soundness of Actris 2.0 is proven using a model of its protocol mechanism in the Iris framework. We have mechanised the theory of Actris, together with custom tactics, as well as all examples in the paper, in the Coq proof assistant.

==> lstcoq.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{coq} {
% Comments may or not include Latex commands
texcl=false,

% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Add, Morphism, Relation,
Implicit, Arguments, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Context, Class, Global, Instance, Program, Infix,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Extern, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside, Eval,
Check},

% Gallina
morekeywords=[2]{forall, exists, exists2, fun, fix, cofix,
      match, %with, end, %as,
      %in, return, % let, is,
      if, then, else,
      %for, %of,
      nosimpl},

% Sorts
morekeywords=[3]{Set, Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
%morekeywords=[4]{
%         pose, set, move, case, elim, apply, clear,
%            hnf, intro, intros, generalize, rename, pattern, after,
%	    destruct, induction, using, refine, inversion, injection,
%         rewrite, congr, unlock, compute, field, fourier,
%            replace, fold, unfold, change, cutrewrite, simpl,
%         have, suff, wlog, suffices, without, loss, nat_norm,
%            assert, cut, trivial, revert, bool_congr, nat_congr,
%	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
%morekeywords=[5]{
%         by, done, exact, tauto, romega, omega,
%         assumption, solve, contradiction, discriminate},


% Control
%morekeywords=[6]{do, last, first, try, idtac, repeat},

morestring=[b]{"},

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% Size of tabulations
tabsize=3,							

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style for listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\bfseries\color{red}},
keywordstyle=[2]{\ttfamily\bfseries\color{blue}},
keywordstyle=[3]{\ttfamily\bfseries},

%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\color{blue}},

moredelim=[is][\color{black}]{@@}{@},
}

